Markovian Score Climbing: Variational Inference with KL(p||q)

Modern variational inference (VI) uses stochastic gradients to avoid intractable expectations, enabling large-scale probabilistic inference in complex models. VI posits a family of approximating distributions q and then finds the member of that family that is closest to the exact posterior p. Traditionally, VI algorithms minimize the "exclusive Kullback-Leibler (KL)" KL(q || p), often for computational convenience. Recent research, however, has also focused on the "inclusive KL" KL(p || q), which has good statistical properties that makes it more appropriate for certain inference problems. This paper develops a simple algorithm for reliably minimizing the inclusive KL using stochastic gradients with vanishing bias. This method, which we call Markovian score climbing (MSC), converges to a local optimum of the inclusive KL. It does not suffer from the systematic errors inherent in existing methods, such as Reweighted Wake-Sleep and Neural Adaptive Sequential Monte Carlo, which lead to bias in their final estimates. We illustrate convergence on a toy model and demonstrate the utility of MSC on Bayesian probit regression for classification as well as a stochastic volatility model for financial data.

==> preamble.tex <==
\RequirePackage[l2tabu, orthodox]{nag}

% GENERAL
\usepackage{enumerate}
\usepackage[inline]{enumitem}

% FONTS
\usepackage[T1]{fontenc}

% Replace default Latin Modern typewriter with its proportional counterpart
% http://www.tug.dk/FontCatalogue/lmoderntypewriterprop/
\renewcommand*\ttdefault{lmvtt}


%%% OPTION 1 - Fourier Math + New Century Schoolbook + ParaType Sans

% % Import Fourier Math (this imposes its own New Century Schoolbook type)
% % http://www.ctan.org/tex-archive/fonts/fouriernc/
% \usepackage{fouriernc}
% \usepackage{amsmath}
% % Replace with TeX Gyre Schola version of New Century Schoolbook (must scale!)
% % http://www.tug.dk/FontCatalogue/tgschola/
% \usepackage[scale=0.92]{tgschola}
% \usepackage[scaled=0.88]{PTSans}

%% OPTION 2 - MathDesign Math + Bitstream Charter + ParaType Sans

% Import MathDesign (this brings along Bitstream Charter)
% http://www.ctan.org/tex-archive/fonts/mathdesign/
\usepackage[bitstream-charter]{mathdesign}
\usepackage{amsmath}
\usepackage{amsthm}
%\usepackage[scaled=0.92]{PTSans}
\usepackage{dsfont}

% %%% OPTION 3 - MTPRO 2 Math + Termes Times + ParaType Sans

% \usepackage{tgtermes}
% \usepackage{amsmath}
% \usepackage[subscriptcorrection,
%             amssymbols,
%             mtpbb,
%             mtpcal,
%             nofontinfo  % suppresses all warnings
%            ]{mtpro2}
% \usepackage{scalefnt,letltxmacro}
% \LetLtxMacro{\oldtextsc}{\textsc}
% \renewcommand{\textsc}[1]{\oldtextsc{\scalefont{1.10}#1}}
% \usepackage[scaled=0.92]{PTSans}

% GEOMETRY
%\usepackage[
%  paper  = letterpaper,
%  left   = 1.65in,
%  right  = 1.65in,
%  top    = 1.0in,
%  bottom = 1.0in,
%  ]{geometry}

% COLOR
\usepackage[usenames,dvipsnames]{xcolor}
\definecolor{shadecolor}{gray}{0.9}

% SPACING and TEXT
%\usepackage[final,expansion=alltext]{microtype}
\usepackage[english]{babel}
\usepackage[parfill]{parskip}
\usepackage{afterpage}
\usepackage{framed}

\usepackage{nicefrac}       % compact symbols for 1/2, etc.

%redefine the leftbar environment to accept a width and coloring options
\renewenvironment{leftbar}[1][\hsize]
{%
  \def\FrameCommand
  {%
    {\color{Gray}\vrule width 3pt}%
    \hspace{10pt}%
    %\hspace{0pt}\fboxsep=\FrameSep\colorbox{black!10}%
  }%
  \MakeFramed{\hsize#1\advance\hsize-\width\FrameRestore}%
}%
{\endMakeFramed}

% define a paragraph header function
\DeclareRobustCommand{\parhead}[1]{\textbf{#1}~}

% EDITING
% line numbering in left margin
\usepackage{lineno}
\renewcommand\linenumberfont{\normalfont
                             \footnotesize
                             \sffamily
                             \color{SkyBlue}}
% ragged paragraphs in right margin
\usepackage{ragged2e}
\DeclareRobustCommand{\sidenote}[1]{\marginpar{
                                    \RaggedRight
                                    \textcolor{Plum}{\textsf{#1}}}}
% paragraph counter in right margin
\newcommand{\parnum}{\bfseries\P\arabic{parcount}}
\newcounter{parcount}
\newcommand\p{%
    \stepcounter{parcount}%
    \leavevmode\marginpar[\hfill\parnum]{\parnum}%
}
% paragraph helper
\DeclareRobustCommand{\PP}{\textcolor{Plum}{\P} }

% COUNTERS
\renewcommand{\labelenumi}{\color{black!67}{\arabic{enumi}.}}
\renewcommand{\labelenumii}{{\color{black!67}(\alph{enumii})}}
\renewcommand{\labelitemi}{{\color{black!67}\textbullet}}

% FIGURES
\usepackage{graphicx}
\usepackage[labelfont=bf]{caption}
\usepackage[format=hang]{subcaption}
\usepackage{wrapfig}

% TABLES
\usepackage{booktabs}

% ALGORITHMS
\usepackage[algoruled,linesnumbered]{algorithm2e}
\usepackage{listings}
\usepackage{fancyvrb}
\fvset{fontsize=\normalsize}

% BIBLIOGRAPHY
%\usepackage[numbers]{natbib}

% HYPERREF
\usepackage[colorlinks,linktoc=all]{hyperref}
\usepackage[all]{hypcap}
\hypersetup{citecolor=BurntOrange}
\hypersetup{linkcolor=MidnightBlue}
\hypersetup{urlcolor=MidnightBlue}

% CLEVEREF must come after HYPERREF
\usepackage[nameinlink]{cleveref}

% ACRONYMS
\usepackage[acronym,nowarn,smallcaps]{glossaries}
%\usepackage[acronym,nowarn]{glossaries}
% \makeglossaries

% COLOR DEFINITIONS
\newcommand{\red}[1]{\textcolor{BrickRed}{#1}}
\newcommand{\orange}[1]{\textcolor{BurntOrange}{#1}}
\newcommand{\green}[1]{\textcolor{OliveGreen}{#1}}
\newcommand{\blue}[1]{\textcolor{MidnightBlue}{#1}}
\newcommand{\gray}[1]{\textcolor{black!60}{#1}}

% LISTINGS DEFINTIONS
\lstdefinestyle{mystyle}{
    commentstyle=\color{OliveGreen},
    keywordstyle=\color{BurntOrange},
    numberstyle=\tiny\color{black!60},
    stringstyle=\color{MidnightBlue},
    basicstyle=\ttfamily,
    breakatwhitespace=false,
    breaklines=true,
    captionpos=b,
    keepspaces=true,
    numbers=left,
    numbersep=5pt,
    showspaces=false,
    showstringspaces=false,
    showtabs=false,
    tabsize=2
}
\lstset{style=mystyle}


==> preamble_tikz.tex <==
\usepackage{tikz}
% \usetikzlibrary{bayesnet}

\pgfdeclarelayer{edgelayer}
\pgfdeclarelayer{nodelayer}
\pgfsetlayers{edgelayer,nodelayer,main}

\definecolor{hexcolor0xbfbfbf}{rgb}{0.749,0.749,0.749}

\tikzset{>=latex}
\tikzstyle{none}   = [inner sep=0pt]

\tikzstyle{line}  = [ - ]
\tikzstyle{arrow}  = [ ->, shorten <=1pt, shorten >=1pt ]
\tikzstyle{ardash} = [ dotted, ->, shorten <=1pt, shorten >=1pt ]

\tikzstyle{empty}=[circle,opacity=0.0,text opacity=1.0,inner sep=0pt,minimum
width=0pt,minimum height=0pt]
\tikzstyle{box}=[rectangle,fill=White,draw=Black]
\tikzstyle{filled}=[circle,fill=hexcolor0xbfbfbf,draw=Black]
\tikzstyle{hollow}=[circle,fill=White,draw=Black]
\tikzstyle{param}=[rectangle,fill=Black,draw=Black,inner sep=0pt,minimum width=4pt,minimum height=4pt]


==> sec_biased.tex <==
\section{Biased Stochastic Approximation and Its Consequences}\label{sec:biased}
The key idea in stochastic gradient descent for \gls{VI} is to estimate the gradient of the objective function using random numbers, often based on \gls{MC} methods. If the objective function is the commonly used exclusive \gls{KL} divergence $\textrm{KL}(q(\latent\idxby \varparams) \| p(\latent\given\data) )$, \ie from the variational approximation $q$ to the posterior $p$, we can make use of score function gradient estimators \citep{Paisley2012,Salimans2013,Ranganath2014}, reparameterization gradient estimators  \citep{Rezende2014,Kingma2014}, or a combination of the two \citep{Ruiz2016,Naesseth2017}. These methods ensure unbiased stochastic gradients that results in an iterative \gls{SA} algorithm that convergences to a local optima of the exclusive \gls{KL} divergence. However, when considering the \emph{inclusive} \gls{KL} the solution is less clear. Both \citet{gu2015neural} and \citet{Bornschein2015} resort to biased (self-normalized) \gls{IS} and \gls{SMC} approximations of the gradients for optimizing the variational parameters. 

%Another issue is that data subsampling is less straightforward when considering the inclusive \gls{KL}. One solution is to follow \citet{li2016renyi,dieng2017chi} where the authors propose to replace the likelihood with a subsampled (geometric) average. Both these approaches introduce a non-vanishing systematic bias to the gradients, resulting in a fixed point that is not a local optima of the inclusive \gls{KL}. 
Below we study this bias and its impact on the optimized variational approximation. In \cref{sec:method} we will show how to resolve the issue by using \gls{SA} algorithms based on gradients estimated with \gls{MCMC}.

\subsection*{Estimating the Gradient using Importance Sampling}\label{sec:biased:is}
The gradient with respect to the variational parameters of the objective function in \cref{eq:kloptproblem} is intractable. However, it is possible to derive an unbiased gradient based on \gls{IS} \citep{robert2013monte}, rewriting the gradient as an expectation with respect to $q$. The gradient of the inclusive \gls{KL} is proportional to
\begin{align}
	\grad_\varparams L_{\textrm{KL}}(\varparams) &\propto \Exp_{ q(\latent\idxby \varparams) } \left[-\frac{p(\latent,\data)}{q(\latent\idxby \varparams)} \grad_\varparams \log  q(\latent\idxby \varparams) \right],
\end{align}
where the constant of proportionality $\nicefrac{1}{p(\data)}$ is independent of the variational parameters and will not affect the solution of the corresponding fixed point equation. Unfortunately, while unbiased, estimating this gradient using standard \gls{MC} methods can lead to high variance. \citet{gu2015neural} and \citet{Bornschein2015}\footnote{specifically the so called \emph{wake update}}, instead propose to make use of the following self-normalized \gls{IS} (or corresponding \gls{SMC}) estimate
\begin{align}
	\grad_\varparams L_{\textrm{KL}}(\varparams) &\approx - \sum_{s=1}^S \frac{w_s}{\sum_{r=1}^S w_r}\grad_\varparams \log  q(\latent^s \idxby \varparams) , \label{eq:sgd:inclkl}
\end{align}
where $w_s = \frac{p(\latent^s,\data)}{q(\latent^s\idxby \varparams)}$ and $\latent^s \sim q(\latent^s \idxby \varparams)$. While this approach decreases the variance of the gradient estimator it also introduces a systematic error; the estimator is no longer unbiased and as a result the variational parameters achieved are no longer optimal \wrt the original minimization problem in \cref{eq:divoptproblem}. For a thorough introduction and treatment of \gls{IS} and \gls{SMC} methods we refer the reader to \eg \citet{naesseth2019elements,mcbook}.

\subsection*{Empirical Illustration of the Bias}\label{sec:biased:is:expts}
We illustrate the bias in the optimal parameters on a toy example. Let $p(\latent\given\data)$ be a scalar skew normal distribution with location, scale and shape parameters $(\xi, \omega, \alpha) = (0.5, 2, 5)$. We let the variational approximation be a family of normal distributions $q(\latent\idxby \varparams) = \Norm(\latent\idxby \mu, \sigma^2)$. For this choice of posterior and approximating family it is possible to compute the analytical solution for the inclusive \gls{KL} divergence; it corresponds to matching the moments of the variational approximation and the posterior distribution. %To compute the true solution for the $\chi^2$ divergence we use the mean of $- \nicefrac{p(\latent,\data)}{q(\latent\idxby \varparams)} \grad_\varparams \log q(\latent\idxby \varparams)$ based on a thousand samples from $p(\latent\given\data)$ at each iteration. 
In \cref{fig:biased} we show the results of \gls{SGD} when using the biased gradients from \cref{eq:sgd:inclkl}, \ie using self-normalized \gls{IS} to estimate the gradients, and \gls{MSC} (this paper) as described in \cref{sec:method}. We set the number of samples to $S=2$. We can see how the biased gradient leads to systematic errors when estimating the variational parameters, whereas \gls{MSC} obtains the true solution. While increasing the number of samples for the estimator in \cref{eq:sgd:inclkl} will lower the bias, and in the limit of infinite samples $S$ it is exact, this is clearly impractical. % However, the estimator in \cref{eq:sgd:chisquared} is biased even as $S\to \infty$. 
\begin{figure}[h]
	\centering
	\begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{skewnormal_inclkl_mean}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[width=\textwidth]{skewnormal_inclkl_logsigma}
    \end{subfigure}
	\caption{Example of learnt variational parameters for \gls{IS}- and \gls{MSC}-based gradients of the inclusive \gls{KL}, as well as true parameters.  The example uses a Gaussian approximation to a skew normal posterior distribution. Iterations in log-scale.}\label{fig:biased}
\end{figure}

A similar bias is also present in the gradients for R\'{e}nyi- and $\chi$ divergences used in \eg \citet{li2016renyi,dieng2017chi}. This will likewise lead to a systematic error in the optimal solution, \ie the optimal variational parameter obtained is \emph{not a local optima} to the original optimization problem. We provide a $\chi$ divergence analogue to \cref{fig:biased} in the supplementary material to illustrate this point.

In \cref{sec:method} we show how it is possible to construct stochastic gradients for the inclusive \gls{KL} that ensure convergence to a local optima of the inclusive \gls{KL} \cref{eq:divoptproblem}, even while the number of samples $S$ at each step is finite.




